CO2-rich protoplanetary discs as a probe of dust radial drift & trapping

MIR spectra imply considerable chemical diversity in the inner regions of protoplanetary discs: some are H2O-dominated, others by CO2. Sublimating ices from radially drifting dust grains are often invoked to explain some of this diversity, particularly the H2O-rich discs. We use a 1D protoplanetary disc evolution code to model how radially drifting dust grains that transport ices inwards to snowlines impact the chemistry of the inner regions of protoplanetary discs. We explore differences between smooth discs and those where radial drift is impeded by dust trapping outside gas gaps and quantify the effects of gap location and formation time. Discs evolve through an initial H2O-rich phase due to sublimating ices, followed by a CO2-rich phase as H2O vapour advects onto the star and CO2 advects into the inner disc from its snowline. The inclusion of traps hastens the transition between the phases, raising the CO2/H2O ratio; gaps opened early or close-in produce lower increases by blocking more CO2 ice from reaching the inner disc. This leads to a potential correlation between CO2/H2O and gap location that occurs on Myr timescales for fiducial parameters. We produce synthetic spectra from the models which we analyse with 0D LTE slab models to understand how this evolution may be expressed observationally. Whether the evolution can be retrieved depends on the contribution of dust grains to the optical depth: dust that couples to the gas after crossing the H2O snowline can add to the continuum optical depth and obscure the delivered H2O, largely hiding the evolution in its visible column density. However, the CO2/H2O visible column density ratio is only weakly sensitive to dust continuum obscuration. This suggests it may be a clearer tracer of the impact of transport on chemistry than individual column densities for spectra that show weak features probing deep enough in the disc. (Abridged)

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
